Workload-Aware Incremental Reclustering in Cloud Data Warehouses

Modern cloud data warehouses store data in micro-partitions and rely on metadata (e.g., zonemaps) for efficient data pruning during query processing. Maintaining data clustering in a large-scale table is crucial for effective data pruning. Existing automatic clustering approaches lack the flexibility required in dynamic cloud environments with continuous data ingestion and evolving workloads. This paper advocates a clean separation between reclustering policy and clustering-key selection. We introduce the concept of boundary micro-partitions that sit on the boundary of query ranges. We then present WAIR, a workload-aware algorithm to identify and recluster only boundary micro-partitions most critical for pruning efficiency. WAIR achieves near-optimal (with respect to fully sorted table layouts) query performance but incurs significantly lower reclustering cost with a theoretical upper bound. We further implement the algorithm into a prototype reclustering service and evaluate on standard benchmarks (TPC-H, DSB) and a real-world workload. Results show that WAIR improves query performance and reduces the overall cost compared to existing solutions.

==> 0-letter.tex <==
\thispagestyle{empty}

\renewcommand{\thefigure}{R\arabic{figure}}
\renewcommand{\thealgorithm}{R\arabic{algorithm}}

We sincerely thank the reviewers for their constructive feedback and the opportunity to revise our manuscript.
We have carefully addressed the major concerns regarding experimental evaluation and workload diversity in the following four main modifications.
Please refer to ``MAJOR COMPONENTS'' for the full elaboration.

\begin{enumerate}[leftmargin=*]
    \item
          \textbf{Complex Workloads (Meta, R1, R4)}. We integrated the DSB benchmark into our evaluation in \underline{\cref{sec:dsb}}.
          Experimental results (\underline{\smash{\cref{fig:overall,fig:dsb}}}) show a 60.3\% cost reduction for \algname and confirm that WAIR robustly outperforms baselines over time in data warehousing workloads involving complex query types (e.g., JOINs) and diverse predicates in \underline{\cref{sec:dsb-eval}}.
    \item \textbf{Workload Generator (R1)}.
          We developed a configurable workload generator in \underline{\cref{sec:workload-generator}} to extend synthetic benchmarks into continuous, time-varying streams.
          This generator enables parameter-controlled evaluation of pruning techniques.
    \item \textbf{Robustness \& Sensitivity (Meta, R1, R4)}. Leveraging the workload generator, we conducted a systematic sensitivity analysis in \underline{\cref{sec:tpc-h-eval,sec:dsb-eval}} by varying environmental parameters.
          These results (\underline{\smash{\cref{fig:sensitivity}}}) trace how each approach responds to parameter changes.
          We also extended our theoretical analysis to derive amortized cost bounds under clustering key shifts and system constraints in \underline{\cref{sec:adjustments}}.
    \item \textbf{Cost Model Extensions (R1)}. We extended \algname's standard cost model to demonstrate user-specific control over reclustering aggressiveness and budget constraints in \underline{\cref{sec:extensions}} and empirically evaluated in \underline{\smash{\cref{fig:aggressive}}}.
          We further included a discussion on how to generalize the framework to incorporate the interplay with query performance in \underline{\cref{sec:extensions}}.
\end{enumerate}

We standardized the presentation of results across workloads: end-to-end results, followed by breakdowns and  sensitivity analyses (\underline{\cref{sec:end-to-end,sec:tpc-h-eval,sec:dsb-eval,sec:mirrors-eval}}).
We also expanded the discussions on related work (\underline{\cref{sec:related}}), implementation on distributed engines (\underline{\cref{sec:distributed}}), pruning opportunities (\underline{\cref{sec:pruning}}), evaluation metrics (\underline{\cref{sec:setup}}), and real-world dataset analysis (\underline{\cref{sec:mirrors-eval}}).
In addition, we revised the text in the paper thoroughly to incorporate the reviewers' detailed editorial suggestions.

\smallskip
We highlight the changes in the revision as:
\begin{enumerate}[label=--, leftmargin=*]
    \item \textbf{\color{blue} Blue}: Common major changes and new experiments.
    \item \textbf{\color{DarkGreen} Green}: Responses to Reviewer \#1.
    \item \textbf{\color{orange} Orange}: Responses to Reviewer \#3.
    \item \textbf{\color{purple} Purple}: Responses to Reviewer \#4.
\end{enumerate}

\section*{RESPONSE TO META-REVIEWER}

\begin{reviewercomment}
    \textbf{Revision Item 1}\ \ Include at least one ``complex'' data warehousing workload such as TPC-DS or DSB.
\end{reviewercomment}
\noindent\textbf{Response:} We added the DSB benchmark (derived from TPC-DS) into our evaluation.
Please refer to \textbf{Added Component 1}.

\begin{reviewercomment}
    \textbf{Revision Item 2}\ \ Preferably one other dataset/workload (e.g., a real-world dataset/workload) if possible.
\end{reviewercomment}
\noindent\textbf{Response:} We previously included a real-world dataset (Mirrors) in our evaluation and now expanded its result analysis (\underline{\cref{sec:mirrors-eval}}).
In addition, we developed a configurable workload generator to produce diverse scenarios beyond static benchmarks in \textbf{Added Component 2}.
We then used it to conduct a systematic sensitivity analysis to evaluate the performance and robustness of \algname and the baselines across these workloads in \textbf{Added Component 3}.
These additional evaluations further confirm \algname's effectiveness to complex workloads.

\begin{reviewercomment}
    \textbf{Revision Item 3}\ \ Address all issues raised by the reviewers.
\end{reviewercomment}
\noindent\textbf{Response:} Each point raised by the reviewers has been carefully addressed. Please refer to our detailed responses to each reviewer.

\section*{MAJOR COMPONENTS}
\begin{reviewercomment}
    \textbf{Added Component 1}\ \ Evaluation on DSB benchmark.
\end{reviewercomment}
\noindent\textbf{Description:}
We added DSB (derived from TPC-DS) in our evaluation as requested.
DSB has a more complex schema with multiple fact tables and query templates that target complex joins, numerous filters across diverse columns, and varied aggregations.
At a high level, \algname's reclustering is driven by filtered table scans.
Complex operators that result in filtered range scans (e.g., JOINs) naturally benefit from table clustering.
\algname handles diverse predicates via savings signatures and hybrid layouts that identify the most relevant columns across access patterns.
On DSB,
\algname reduces total cost by 60.3\%, I/O volume by 63.9\%, and outperforms all baselines over time.
Together with a systematic sensitivity analysis in \textbf{Added Component 3} below, these results confirm \algname's effectiveness to complex data warehousing workloads in diverse scenarios.

\smallskip
\noindent\textbf{References:}
\underline{\smash{\cref{fig:overall}}}, \underline{\smash{\cref{fig:dsb}}}, \underline{\cref{sec:dsb}}, \underline{\cref{sec:dsb-eval}}.


\begin{reviewercomment}
    \textbf{Added Component 2}\ \ Configurable Workload Generator.
\end{reviewercomment}
\noindent\textbf{Description:}
Standard benchmarks (e.g., TPC-H) largely rely on static datasets with fixed query templates and limited dynamic features.
Prior evaluations often randomly permute queries on a static snapshot (e.g., Qd-tree \cite{DBLP:conf/sigmod/YangCWGLMLKA20}), which misses the interplay between continuous ingestion and evolving workloads.

To close this gap, we extend our evaluations into a configurable workload generator.
Following our earlier evaluation setup, the generator segments time into batches and periods and models the joint evolution of data ingestion and query workloads.
Standard benchmarks are then extended into continuous, time-varying streams with parameterized control over workload dynamics.
The workload generator underpins a unified evaluation framework and serves as a reusable contribution for both our sensitivity analysis and future research on partition pruning techniques.

\smallskip
\noindent\textbf{Reference:}
\underline{\cref{sec:workload-generator}}.

\begin{reviewercomment}
    \textbf{Added Component 3}\ \ Sensitivity Analysis under Diverse Workloads and Theoretical Analysis.
\end{reviewercomment}
\noindent\textbf{Description:}
We conduct a systematic sensitivity analysis, varying one parameter at a time while keeping the others at their default values.
We examine reclustering start time, workload shifting rate, workload skewness, predicate column diversity, and query selectivity.
\algname remains relatively robust while baselines show varying sensitivity and reveal several trends.
For example, a full table repartitioning (e.g., Qd-tree) can be preferable with a large unordered historical pool and a stable workload.

We also address stability under workload shifts.
We extend our theory to bound the cost under key changes and diverse constraints, mitigating concerns about oscillation.
We show that the adjusted greedy algorithm has an amortized worst-case $O(\log n)$ overhead even when the clustering key changes.
Our empirical hybrid-layout technique likewise shows consistent gains across varied workloads.

\smallskip
\noindent\textbf{References:}
\underline{\smash{\cref{fig:sensitivity}}}, \underline{\cref{sec:adjustments}}, \underline{\cref{sec:tpc-h-eval}}, \underline{\cref{sec:dsb-eval}}.

\begin{reviewercomment}
    \textbf{Added Component 4}\ \ Cost Model Extensions.
\end{reviewercomment}
\noindent\textbf{Description:}
We value the reviewers' suggestion to support user-specific needs to tailor reclustering policies.
Our framework is flexible and supports extensions to the cost model.
We present two such extensions to highlight this flexibility.

First, we add an aggressiveness factor $\alpha$ and a long-term credit mechanism.
These let users control how aggressively to recluster and how strictly to enforce a budget over time.
This extension inherits the theoretical bounds of the adjusted greedy algorithm in \underline{Section 3.3}.
In our evaluation, the more aggressive variant shows similar cost reductions with greater volatility, so we recommend the standard settings.
Second, we propose a price parameter $\beta$ that lets users express how much they value performance improvements. For complex applications, users can also supply custom utility functions to align the cost model with their specific priorities.

\smallskip
\noindent\textbf{References:}
\underline{\smash{\cref{fig:aggressive}}}, \underline{\cref{sec:adjustments}}, \underline{\cref{sec:extensions}}, \underline{\cref{sec:ablation}}.


\section*{RESPONSE TO REVIEWER \#1}

\begin{reviewercomment}
    \textbf{R1.O1.1}\ \ The experimental workload is simplified compared to real-world workloads that might also include LIMIT queries, JOINs, and filters on diverse predicates. The paper's evaluation should also address filters on multiple (potentially correlated) attributes.
\end{reviewercomment}
\noindent\textbf{Response:} We addressed this concern in \textbf{Added Component 1}.
In addition, we conducted a sensitivity analysis of predicate column diversity per query in \textbf{Added Component 3}.
These evaluations confirm \algname's applicability to complex workloads.

\begin{reviewercomment}
    \textbf{R1.O1.2}\ \ The paper should also give an overview of pruning possibilities in general.
\end{reviewercomment}
\noindent\textbf{Response:} We added \underline{\cref{sec:pruning}} to outline an overview of pruning opportunities.
In general, queries that result in filtered range scans naturally benefit from table clustering.

\begin{reviewercomment}
    \textbf{R1.O1.3}\ \ An idea could be a workload generator for partition pruning, which might be valuable for future work.
\end{reviewercomment}
\noindent\textbf{Response:}
We sincerely thank the reviewer for this valuable suggestion.
We addressed this in \textbf{Added Component 2}.
The workload generator underpins our following sensitivity analysis in \textbf{Added Component 3} and provides a unified, reusable tool for future research on partition pruning techniques.

\begin{reviewercomment}
    \textbf{R1.O2}\ \ Please make the calculation of the pruning ratio also executable on local machines with minimal dependencies.
\end{reviewercomment}

\begin{algorithm}[t!]
    \caption{IP Address Anonymization for Mirrors Dataset}
    \label{alg:anonymize}
    \begin{algorithmic}[1]
        \Require $secret$ (binary secret key), $mask\_len$ (IPv4: 24; IPv6: 48), $step\_time$ (30 seconds), $ip$ (visitor address)
        \Ensure $h$ (anonymized address)
        \State $len \gets \Call{BitLength}{ip}$ \Comment{IPv4: 32; IPv6: 128}
        \State $t \gets \left\lfloor \Call{UnixTime}{ } \ /\  step\_time \right\rfloor$
        \State $buf \gets \Call{Encode}{ip} \ \Vert\  \Call{UInt32BE}{t \bmod 2^{32}}$
        \State $h \gets \Call{HMAC-SHA1}{secret, buf}[:len]$
        \State $h[:mask\_len] \gets \texttt{ip}[:mask\_len]$
        \State \Return $\Call{Decode}{h}$
    \end{algorithmic}
\end{algorithm}

\noindent\textbf{Response:} During the interactive discussion phase, we updated our artifact repository to include a pipeline and instructions for verifying the algorithm's logic and pruning statistics on local machines with minimal dependencies.

Most importantly, we packaged the workload generator as a standalone, configurable module\footnote{https://github.com/sigmod-26-1209/wg} for community reuse.
For real-world scenarios (Mirrors) where internal workloads cannot be publicly shared, we managed to anonymize and release\footnote{To preserve double-blind review, the repository currently includes a small sample. A public link to the anonymized data will be provided in the final version.} the underlying dataset for the open-source community in \Cref{alg:anonymize}.
The algorithm preserves the network prefix of each IP address and anonymizes its host suffix.
It also maintains the timely correlation of visits from the same user within a time window ($step\_time$).

\begin{reviewercomment}
    \textbf{R1.O3}\ \ Discuss if the pruning rate would be a more suitable metric, which could be ``translated'' into performance and costs.
\end{reviewercomment}

\noindent\textbf{Response:}
We added I/O volume as a complementary metric in \underline{\smash{\cref{fig:overall}}} to capture overall pruning effectiveness.
We choose CPU time as a \textit{unifying metric} to assess end-to-end trade-offs between query execution and reclustering.
While instantiated as CPU time in our experiments, this end-to-end metric generalizes to other cloud environments by platform-specific cost models.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/evaluation/polyfit}
    \caption{Relationship Between Pruning Rate and Query Runtime.
        \textmd{Each point represents a batch's pruning rate and its corresponding normalized scan cost (I/O runtime divided by table size) in TPC-H. The line shows a polynomial fit ($R^2=0.996$).}}
    \Description{Relation Between Pruning Rate and Query Runtime.}
    \label{fig:polyfit}
\end{figure}

From a query-centric perspective, we fully agree that pruning rate is a suitable, system-independent metric for I/O performance.
The pruning rate and normalized scan cost exhibit a strong polynomial relationship in \Cref{fig:polyfit}, confirming that query runtimes are highly correlated with pruning rates in our experiments.
For the sensitivity analysis (\underline{\smash{\cref{fig:sensitivity}}}), we use the average partition pruning rate as a \textit{direct proxy} for query cost to isolate the effect of each parameter in a wide range of workload scenarios.

\begin{reviewercomment}
    \textbf{R1.O4.1}\ \ Outline under which circumstances which approach performs best, and what the break-even points are.
\end{reviewercomment}
\noindent\textbf{Response:} We sincerely thank the reviewer for this valuable suggestion.
We conducted a systematic sensitivity analysis in \textbf{Added Component 3}.
This analysis further confirms \algname's applicability to complex workloads and reveals trends between baselines.

\begin{reviewercomment}
    \textbf{R1.O4.2}\ \ Discuss the interplay of pruning rate, performance, and costs. Consider performing clustering in the background using additional machines at higher costs for better performance.
\end{reviewercomment}
\noindent\textbf{Response:} We addressed this in \textbf{Added Component 4}.
These two extensions further demonstrate the flexibility of our framework to accommodate user-specific needs, including aggressiveness, budget constraints, and performance priorities.


\begin{reviewercomment}
    \textbf{R1.Ms}\ \ Minor remarks.
\end{reviewercomment}
\noindent\textbf{Response:} We thank the reviewer for the careful reading.
We revised the paper to explain ``boundary micro-partitions'' in the \hyperref[sec:abstract]{\underline{Abstract}} and to clarify ambiguous phrasing in \underline{\cref{sec:distributed}}.

\section*{RESPONSE TO REVIEWER \#3}

\begin{reviewercomment}
    \textbf{R3.O1}\ \ Outline an implementation in a distributed engine.
\end{reviewercomment}
\noindent\textbf{Response:} We expanded \underline{\cref{sec:distributed}} to describe how \algname integrates with distributed query engines.
The metadata service seamlessly integrates with a distributed engine's metadata infrastructure as a drop-in component.
Our table-snapshot design enables non-blocking reclustering in distributed settings.
In cloud data warehouses with a cache layer, scan sharing can further reduce reclustering overhead.

\begin{reviewercomment}
    \textbf{R3.O2}\ \ Readability, figures, clarity, and typos.
\end{reviewercomment}
\noindent\textbf{Response:} We sincerely thank the reviewer for the careful reading and the detailed list of minor remarks.
We carefully revised the paper to
improve clarity and overall readability, and placed figures as close as possible to the relevant text.
We also expanded the discussion of the Mirrors workload results in \underline{\cref{sec:mirrors-eval}}.

\smallskip
\noindent \textbf{References:} (M1) \underline{\cref{sec:mirrors-eval}}, (M2) \underline{\cref{tab:flex}}, (M3) \underline{\cref{sec:tpc-h-eval}}, (M4) \underline{\smash{\cref{fig:speed}}}, (M5) \underline{\smash{\cref{fig:overall,fig:tpc-h,fig:centroid,fig:sensitivity,fig:dsb,fig:mirrors,fig:selectivity,fig:speed,fig:aggressive,fig:optimal}}}, (M6) \underline{\smash{\cref{fig:tpc-h}}}.

\section*{RESPONSE TO REVIEWER \#4}

\begin{reviewercomment}
    \textbf{R4.O1.1}\ \ The decision-making algorithms need a broader level of evaluation in order to establish value-add. I would also request evaluation on a corpus with more queries, more tables and richness of predicates beyond TPC-H.
\end{reviewercomment}

\begin{reviewercomment}
    \textbf{R4.O1.2}\ \ I would recommend a control-theoretic stability analysis that articulates why the algorithm will not oscillate.
\end{reviewercomment}

\noindent\textbf{Response:}
We fully acknowledge the reviewer's concern about non-recurrent workload patterns and oscillations under periodic shifts, as well as the request for a stability analysis and a broader evaluation beyond TPC-H.
We address these points both theoretically and empirically, supported by a broader level of evaluation.
\begin{itemize}[leftmargin=*]
    \item \textbf{Theoretical Analysis}: We agree that stability is critical.
          We clarify that our algorithm remains robust even if specific predicates do not occur.
          The analysis of the greedy algorithm in \underline{\cref{sec:greedy}} provides a \textbf{worst-case} logarithmic bound on the cost per operation, which holds regardless of the predicate distribution.
          This ensures the maintenance cost never explodes, even in adversarial scenarios.
          Intuitively, the table's clustering state improves over time, rather than overfitting to single predicates.
          In \underline{\cref{sec:adjustments}}, we further extend the amortized analysis to changing clustering keys in a single-column regime and provide an additional amortized cost of $O(\log n)$.
    \item \textbf{Empirical Practice}:
          In practice, we use a large, self-correcting observation window (\underline{\cref{sec:cost}}) to stabilize reclustering decisions.
          This yields infrequent, high-confidence clustering key switches and further reduces the constant factors in the theoretical bounds.
          Our savings signature framework (\underline{\cref{sec:hybrid}})
          can derive a single global clustering key with the highest aggregated savings to strictly align with theoretical analysis, or leverage our hybrid layout technique for greater flexibility in diverse scenarios.
          In addition, our cost model (\underline{\cref{sec:cost}}) prevents thrashing and ensures that our algorithm does not \emph{undo} previous work unless the predicted benefit explicitly exceeds the reclustering cost.
          This effectively creates a stability buffer, preventing oscillation on short-term noise, as confirmed by a broad level of evaluation.
    \item \textbf{Broader Evaluation}:
          We added the DSB benchmark to our evaluation in \textbf{Added Component 1}.
          DSB features a more complex schema with multiple fact tables and richer query templates than TPC-H.
          In DSB, reclustering targets the three largest fact tables, rather than TPC-H's single largest fact table.
          Moreover, in \textbf{Added Component 2--3}, we developed a configurable workload generator to enable a broader level of evaluation through sensitivity analysis on key environmental parameters.
          Ablation Study in \underline{\cref{sec:ablation}} further shows the effectiveness of our hybrid layout technique in handling diverse predicates.
          Together, these evaluations confirm \algname's applicability to complex workloads and its robustness across diverse scenarios.
\end{itemize}

\begin{reviewercomment}
    \textbf{R4.O2}\ \ In the theoretical analysis, `q' can be a large number. Is the key point of the theoretical analysis that reclustering will be an inexpensive operation perhaps?
\end{reviewercomment}
\noindent\textbf{Response:} We apologize for the confusion, and we revised the theoretical analysis (\underline{\cref{sec:greedy}}) for greater precision, clarity, and extensibility.
We confirm that the key takeaway of the theorem is that the amortized cost of a reclustering operation is \textbf{inexpensive}.

To be precise, $q$ denotes the number of distinct keys being queried, which is upper bounded by both the number of queries executed and the total number of keys in the table.
While $q$ itself can be large, \underline{\smash{\cref{thm:greedy}}} states that every query (and thus two reclusterings) incurs only an additive cost of $O(\log q)$.
This cost is \textbf{logarithmic} in $q$ and small in practice (e.g., $\log_2{10^{12}}\approx 40$), especially relative to the output size.

\begin{reviewercomment}
    \textbf{R4.O3}\ \ The paper makes some assertions that are questionable. For example ``the only reclustering approach that is robust against workload shifts.'' These assertions must be backed by careful reasoning and experiments.
\end{reviewercomment}
\textbf{Response:} We sincerely thank the reviewer for pointing out our potentially risky statements.
In the quoted sentence, our intent was to highlight the experimental results, not to overclaim.
We corrected this wording in \hyperref[sec:abstract]{\underline{Abstract}}.
We also carefully revised throughout the manuscript to remove such bold statements.
Furthermore, we expanded both the theoretical and empirical analyses to better support our claims about robustness under diverse scenarios in \textbf{Added Components 1--3}.

\begin{reviewercomment}
    \textbf{R4.O4}\ \ The treatment of related work is very slim. There have been other reclustering approaches, including some that are learnt, as well as in production with different providers.
\end{reviewercomment}
\textbf{Response:} We thank the reviewer for pointing out the missing literature and the detailed references.
We expanded \underline{\cref{sec:related}} to broaden the discussion of related database techniques and the overloaded term ``partitioning''.
Below is a summary of the position of \algname across the cited references.

\begin{enumerate}[leftmargin=*]
    \item \textbf{Distributed Partitioning (Sharding / Load Balancing).}

          \textit{Goal: Minimize cross-node network traffic and compute skew.}
          \begin{itemize}[leftmargin=*]
              \item \textbf{Horizontal Sharding:} Techniques such as the Distribution Advisor in Azure Synapse SQL \cite{DBLP:journals/pvldb/Aguilar-Saborit20,azure2025distributionadvisor} optimize data placement across nodes (e.g., round-robin vs. hash vs. replicated).
              \item \textbf{Streaming Partitioning:} Approaches like Dalton \cite{DBLP:journals/pvldb/ZapridouMA22} dynamically route tuples in distributed streaming systems to balance loads across operators.
          \end{itemize}
          \textit{Relation to \algname:} \textbf{Orthogonal.} Our work operates at a different system layer and addresses a distinct problem.

    \item \textbf{Micro-Partition Zone Maps (The Context).}

          \textit{Goal: Enable lightweight data skipping on cloud object stores.}
          \begin{itemize}[leftmargin=*]
              \item \textbf{Data Skipping Paradigm:} Cloud Data Warehouses (e.g., Snowflake \cite{DBLP:conf/sigmod/DagevilleCZAABC16, DBLP:conf/sigmod/ZimmererDKWOK25}) store data in micro-partitions on object stores (e.g., S3) and favor lightweight min-max zone maps \cite{DBLP:journals/pvldb/ZiauddinWKLPK17} over heavy indexing (e.g, B-Trees).
              \item \textbf{Locality Preservation:} Multi-dimensional space-filling curves (e.g., Z-ordering \cite{DBLP:conf/sigmod/Orenstein86}, Hilbert curves \cite{DBLP:journals/tc/Butz71}) are the standard practice to preserve locality across multiple columns, enabling zone maps to function effectively.
          \end{itemize}

          \textit{Relation to \algname:} \textbf{Foundational.} \algname operates strictly within this data-skipping paradigm to maximize zone maps efficacy.

    \item \textbf{Table Layout Optimization (The Core).}

          \textit{Goal: Organize records across micro-partitions to optimize table clustering state and pruning efficiency.}
          \begin{itemize}[leftmargin=*]
              \item \textbf{Static Layouts:} Learned layouts (e.g., Qd-tree \cite{DBLP:conf/sigmod/YangCWGLMLKA20}) optimize for specific query workloads but typically require expensive full rewrites and target static snapshots.
              \item \textbf{Reclustering:} We provide in \underline{\cref{sec:related}} a comprehensive taxonomy of existing table reclustering methods and their limitations in dynamic workload scenarios.
                    Notably, Snowflake's Automatic Clustering \cite{ac} (also adopted by Dremio \cite{dmaic}) is essentially the \textit{data-driven} baseline and evaluated as \textbf{DD} in our experiments.
                    \algname goes beyond the static metrics to optimize for dynamic workloads.
          \end{itemize}
          \textit{Relation to \algname:} \textbf{Advancement.} We advance this category by a cost-based, workload-aware algorithm and framework to maintain table clustering state under dynamic scenarios.
\end{enumerate}


With these distinctions in mind, we clarify and summarize our key contributions as follows:

\begin{enumerate}[leftmargin=*]
    \item a policy-key decoupled taxonomy and framework for the table clustering problem (\underline{\cref{sec:preliminaries}}),
    \item the notion of boundary micro-partitions and the logarithmic theoretical upper bound on the amortized cost of reclustering them under workload shifts and diverse constraints (\underline{\cref{sec:boundary}}),
    \item an adaptive algorithm and framework that efficiently and automatically maintains high-quality table clustering under dynamic workloads (\underline{\cref{sec:wair,sec:ars}}),
    \item a broad level of evaluation and sensitivity analysis across complex workloads and diverse scenarios to analyze the performance and robustness of \algname, its variants, and the baselines in a sound way (\underline{\cref{sec:evaluation}}).
\end{enumerate}
